The Societal Impact of Foundation Models: Advancing Evidence-based AI Policy

Artificial intelligence is humanity's most promising technology because of the remarkable capabilities offered by foundation models. Yet, the same technology brings confusion and consternation: foundation models are poorly understood and they may precipitate a wide array of harms. This dissertation explains how technology and society coevolve in the age of AI, organized around three themes. First, the conceptual framing: the capabilities, risks, and the supply chain that grounds foundation models in the broader economy. Second, the empirical insights that enrich the conceptual foundations: transparency created via evaluations at the model level and indexes at the organization level. Finally, the transition from understanding to action: superior understanding of the societal impact of foundation models advances evidence-based AI policy. View together, this dissertation makes inroads into achieving better societal outcomes in the age of AI by building the scientific foundations and research-policy interface required for better AI governance.

==> acknowledgements_hidden.tex <==
\prefacesection{Acknowledgments}
\todo{First sentence.}

I thank my family for their constant support throughout my research journey. 
My grandmother అమ్మమ్మ embodies warmth, wisdom, and vitality. 
She sets the standard in our family for excellence. The path I have chosen, and the decisions along the way, may not make sense in full to my parents, but they accept that I will find my way through the world. That has not always been easy for them, but I appreciate this as yet another gift they have given me to reach my goals. My confidence to be the person and scholar I want to be without exception begins with the trust I have in them: their sturdy foundation is why I do not fear failure.  

I thank my teachers throughout childhood who fostered my intellectual curiosity and reverence for education, especially Mr. Lozada, Mrs. Gallo, Mrs. Stokrocki, Mrs. Wilson, Mrs. Powers, Mrs. Srinivas, and Mrs. Friedman.\footnote{School teachers who focus on education and university professors who focus on research often feel worlds apart to me. As I acknowledge my teachers, I am reminded that one of AI’s largest societal impacts to date, which I largely did not study in spite of being at an education institution, has been how it warped education. As I often build bridges between otherwise distant groups, I wonder if this AI-driven reckoning should be an invitation to bring these two groups closer. I leave this note to remind myself to reconsider this when I am a professor, drawing inspiration from Rob Reich’s past as a teacher, and to pursue teaching excellence irrespective of institutional incentives, drawing inspiration especially from Percy Liang’s teaching excellence.}  I thank Nivetha Karthikeyan for being better than me at many things but, in particular, her passion for writing and history as well as her broader appreciation for the social sciences and the humanities. While my natural affinity for mathematics led me to get a PhD in computer science, many of my distinctive strengths as a computer scientist were first acquired in my misbegotten attempts to compete with her. Her scholarly defiance continues to inspire me.

\paragraph{College.}
I thank Ravi Ramakrishna and Linus Setiabrata for their childlike love for mathematics. When I arrived at Cornell, I found myself listless. I had lost much of my excitement to learn, and did not what research was. That changed watching them find joy in their study of mathematics. While I quickly realized I could not match their talents, and took the well-trodden path from failed mathematician to computer scientist, I discovered research and rediscovered learning from them.

I thank Bobby Kleinberg, Kavita Bala, Eva Tardos, Lillian Lee, Marty van Schijndel, Vlad Niculae, Xanda Schofield, among others, for their mentorship at Cornell.   I thank Claire Cardie for \todo{insert these ack}. It is only in leaving Cornell that I realize how precious her investment was in me.  Most of all, I thank Arzoo Katiyar: the first paper I ever read was \todo{\citet{}}, the first paper I ever reviewed was with Arzoo’s guidance, and the first paper I ever wrote was with Arzoo \todo{\citep{}}. I may very well have been Arzoo’s first student and I am so sad she cannot be here to read this dissertation. My final memory of Arzoo was her pride in me for getting into grad school: she was more overjoyed than I was. The world cannot be as bright without the light in her eyes to make it brighter.

\paragraph{Transition to Stanford.}
On April 15, 2020, I made the critical decision to come to Stanford over Berkeley. That process introduced me to several folks that I can continue to feel fortunate to share a community with. I thank Dan Klein, because passing on the opportunity to be his student made me certain I had to make the best of my time at Stanford to not regret that decision. I thank Yejin Choi, then for being a friendly face at my first conference (AKBC 2019) where I felt completely out of place , and for having been an ever-wonderful mentor even since. I thank Tatsu Hashimoto, first 


==> reflections.tex <==
\chapter{Reflections}\label{chapter:reflections}
\chaptermark{\small Reflections}

==> tables/downstream.table.tex <==
\begin{table}
\centering
\tiny
\begin{tabular}{l}
Downstream \\
Release decision-making: Does the model developer disclose its protocol for deciding whether or not to release a model? \\
Release process: Does the model developer disclose information related to the process of how the model was released? \\
Distribution channels: Are all distribution channels disclosed?  \\
Products and services: Does the developer disclose whether any products and services offered by the developer are dependent on the model? \\
Machine-generated content: Does the developer disclose whether they have a mechanism for detecting content generated by this model? \\
Model license: For all model assets, is an associated license disclosed?  \\
Terms of service: For all distribution channels, does the distribution channel disclose terms-of-service? \\
Permitted and prohibited users: Does the developer detail who can and cannot use the foundation model?  \\
Permitted, restricted, and prohibited uses: Does the developer disclose a policy that outlines uses of the model that are permitted, restricted, and prohibited?  \\
User interaction with AI system: Across all distribution channels with user-facing interfaces, are users notified that they are interacting with an AI system, the underlying foundation model, and when data is machine-generated? \\
Usage disclaimers: Across all distribution channels with user-facing interfaces, are users notified with relevant disclaimers involving usage?  \\
Usage policy enforcement: Is the enforcement protocol for the usage policy disclosed? \\
Justification for enforcement action: Does the developer give justification to users when they are subject to an enforcement action for violating the usage policy?  \\
Usage policy violation appeals mechanism: Does the developer provide a mechanism for appealing potential usage policy violations?   \\
Permitted, restricted, and prohibited model behaviors: Does the developer disclose a policy that outlines model behavior that is permitted, restricted, and prohibited? \\
Model behavior policy enforcement: Is the enforcement protocol for the model behavior policy disclosed? \\
Interoperability of usage and model behavior policies: Does the model developer disclose how the usage policy and the model behavior policy interoperate? \\
User data protection policy: Does the developer disclose its protocols for storing, accessing, and sharing, and sharing user data?  \\
Permitted and prohibited use of user data: Does the developer disclose its policy for permitted and prohibited uses of user data? \\
Versioning protocol: Is there a disclosed version and versioning protocol for the model? \\
Change log:  Is there a disclosed change log for the model? \\
Deprecation policy: Is there a disclosed deprecation policy for the model developer?  \\
Feedback mechanism: Is a feedback mechanism disclosed? \\
Feedback summary:  Is a report or summary of the feedback the developer received disclosed? Alternatively, is a report or summary of how the developer responded to the feedback disclosed publicly?  \\
Government inquiries: Is a summary of government inquiries received by the developer disclosed? \\
Monitoring mechanism: For all distribution channels, is a monitoring mechanism for tracking model use disclosed? \\
Downstream applications: Across all forms of downstream use, is the number of applications dependent on the foundation model disclosed? \\
Affected market sectors: Across all downstream applications, is the fraction of applications  corresponding to each market sector disclosed?  \\
Affected individuals: Across all forms of downstream use, is the number of individuals affected by the foundation model disclosed?  \\
Usage reports: Does the developer provide a usage report describing the impact of its model on users via usage statistics?  \\
Geographic statistics: Across all forms of downstream use, are statistics of the usage across geographies of the foundation model disclosed?  \\
Redress mechanism: Does the model developer disclose any mechanism to provide redress to users for harm? \\
Usage data access protocol: Is a protocol for granting external entities access to the usage data disclosed?  \\
Centralized documentation for downstream use: Does the developer provide a centralized documentation resource for downstream use? \\
Documentation for responsible downstream use: Does the developer provide documentation for responsible downstream use?    
\end{tabular}
\end{table}
